Performance evaluation of volatility estimation methods for Exabel

Quantifying both historic and future volatility is key in portfolio risk management. This note presents and compares estimation strategies for volatility estimation in an estimation universe consisting on 28 629 unique companies from February 2010 to April 2021, with 858 different portfolios. The estimation methods are compared in terms of how they rank the volatility of the different subsets of portfolios. The overall best performing approach estimates volatility from direct entity returns using a GARCH model for variance estimation.

==> mean_kendall_for_All.long.short_app.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 6 & 0.645 \\ 
  Direct return & GARCH & 12 & 0.645 \\ 
  Direct return & Naive window & 6 & 0.639 \\ 
  Direct return & GARCH & 3 & 0.629 \\ 
  Direct return & Naive window & 12 & 0.624 \\ 
  Direct return & Naive window & 3 & 0.620 \\ 
  Direct return & GARCH & 1 & 0.587 \\ 
  Direct return & Naive window & 1 & 0.573 \\ 
  Factor model & Naive window & 6 & 0.570 \\ 
  Factor model & Naive window & 3 & 0.569 \\ 
  Factor model & GARCH & 6 & 0.569 \\ 
  Factor model & GARCH & 3 & 0.566 \\ 
  Factor model & GARCH & 12 & 0.560 \\ 
  Factor model & Naive window & 12 & 0.556 \\ 
  Factor model & GARCH & 1 & 0.552 \\ 
  Factor model & Naive window & 1 & 0.549 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All long/short'.} 
\label{tab:All.long.short}
\end{table}


==> mean_kendall_for_All.long_app.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.576 \\ 
  Direct return & GARCH & 6 & 0.570 \\ 
  Direct return & GARCH & 3 & 0.558 \\ 
  Direct return & Naive window & 6 & 0.554 \\ 
  Direct return & Naive window & 3 & 0.539 \\ 
  Direct return & Naive window & 12 & 0.539 \\ 
  Direct return & GARCH & 1 & 0.519 \\ 
  Direct return & Naive window & 1 & 0.492 \\ 
  Factor model & GARCH & 6 & 0.470 \\ 
  Factor model & Naive window & 6 & 0.470 \\ 
  Factor model & GARCH & 12 & 0.464 \\ 
  Factor model & GARCH & 3 & 0.463 \\ 
  Factor model & Naive window & 12 & 0.458 \\ 
  Factor model & Naive window & 3 & 0.456 \\ 
  Factor model & GARCH & 1 & 0.434 \\ 
  Factor model & Naive window & 1 & 0.422 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All long'.} 
\label{tab:All.long}
\end{table}


==> mean_kendall_for_All.original.long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.587 \\ 
  Direct return & GARCH & 6 & 0.580 \\ 
  Direct return & GARCH & 3 & 0.568 \\ 
  Direct return & Naive window & 6 & 0.561 \\ 
  Direct return & Naive window & 3 & 0.548 \\ 
  Direct return & Naive window & 12 & 0.546 \\ 
  Direct return & GARCH & 1 & 0.532 \\ 
  Direct return & Naive window & 1 & 0.505 \\ 
  Factor model & GARCH & 6 & 0.471 \\ 
  Factor model & Naive window & 6 & 0.471 \\ 
  Factor model & GARCH & 12 & 0.467 \\ 
  Factor model & GARCH & 3 & 0.464 \\ 
  Factor model & Naive window & 12 & 0.461 \\ 
  Factor model & Naive window & 3 & 0.456 \\ 
  Factor model & GARCH & 1 & 0.435 \\ 
  Factor model & Naive window & 1 & 0.423 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All original long'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:All.original.long}
\end{table}


==> mean_kendall_for_All.original.longshort.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.667 \\ 
  Direct return & GARCH & 6 & 0.665 \\ 
  Direct return & Naive window & 6 & 0.657 \\ 
  Direct return & GARCH & 3 & 0.649 \\ 
  Direct return & Naive window & 12 & 0.642 \\ 
  Direct return & Naive window & 3 & 0.638 \\ 
  Direct return & GARCH & 1 & 0.615 \\ 
  Direct return & Naive window & 1 & 0.601 \\ 
  Factor model & Naive window & 6 & 0.538 \\ 
  Factor model & Naive window & 3 & 0.535 \\ 
  Factor model & GARCH & 6 & 0.533 \\ 
  Factor model & GARCH & 3 & 0.530 \\ 
  Factor model & Naive window & 12 & 0.524 \\ 
  Factor model & GARCH & 12 & 0.522 \\ 
  Factor model & GARCH & 1 & 0.516 \\ 
  Factor model & Naive window & 1 & 0.512 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All original longshort'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:All.original.longshort}
\end{table}


==> mean_kendall_for_All.original.longshort_app.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.667 \\ 
  Direct return & GARCH & 6 & 0.665 \\ 
  Direct return & Naive window & 6 & 0.657 \\ 
  Direct return & GARCH & 3 & 0.649 \\ 
  Direct return & Naive window & 12 & 0.642 \\ 
  Direct return & Naive window & 3 & 0.638 \\ 
  Direct return & GARCH & 1 & 0.615 \\ 
  Direct return & Naive window & 1 & 0.601 \\ 
  Factor model & Naive window & 6 & 0.538 \\ 
  Factor model & Naive window & 3 & 0.535 \\ 
  Factor model & GARCH & 6 & 0.533 \\ 
  Factor model & GARCH & 3 & 0.530 \\ 
  Factor model & Naive window & 12 & 0.524 \\ 
  Factor model & GARCH & 12 & 0.522 \\ 
  Factor model & GARCH & 1 & 0.516 \\ 
  Factor model & Naive window & 1 & 0.512 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All original longshort'.} 
\label{tab:All.original.longshort}
\end{table}


==> mean_kendall_for_All.random.long.short.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & Naive window & 6 & 0.591 \\ 
  Direct return & GARCH & 6 & 0.590 \\ 
  Direct return & GARCH & 12 & 0.590 \\ 
  Direct return & Naive window & 12 & 0.575 \\ 
  Direct return & GARCH & 3 & 0.573 \\ 
  Direct return & Naive window & 3 & 0.569 \\ 
  Direct return & GARCH & 1 & 0.524 \\ 
  Factor model & Naive window & 6 & 0.522 \\ 
  Factor model & GARCH & 6 & 0.521 \\ 
  Factor model & Naive window & 3 & 0.518 \\ 
  Factor model & GARCH & 3 & 0.516 \\ 
  Factor model & GARCH & 12 & 0.511 \\ 
  Direct return & Naive window & 1 & 0.509 \\ 
  Factor model & Naive window & 12 & 0.505 \\ 
  Factor model & GARCH & 1 & 0.498 \\ 
  Factor model & Naive window & 1 & 0.494 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All random long/short'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:All.random.long.short}
\end{table}


==> mean_kendall_for_All.random.long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.570 \\ 
  Direct return & GARCH & 6 & 0.564 \\ 
  Direct return & GARCH & 3 & 0.552 \\ 
  Direct return & Naive window & 6 & 0.550 \\ 
  Direct return & Naive window & 3 & 0.534 \\ 
  Direct return & Naive window & 12 & 0.534 \\ 
  Direct return & GARCH & 1 & 0.511 \\ 
  Direct return & Naive window & 1 & 0.485 \\ 
  Factor model & GARCH & 6 & 0.468 \\ 
  Factor model & Naive window & 6 & 0.468 \\ 
  Factor model & GARCH & 12 & 0.461 \\ 
  Factor model & GARCH & 3 & 0.461 \\ 
  Factor model & Naive window & 12 & 0.455 \\ 
  Factor model & Naive window & 3 & 0.453 \\ 
  Factor model & GARCH & 1 & 0.432 \\ 
  Factor model & Naive window & 1 & 0.419 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All random long'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:All.random.long}
\end{table}


==> mean_kendall_for_All.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.762 \\ 
  Direct return & GARCH & 6 & 0.759 \\ 
  Direct return & Naive window & 6 & 0.751 \\ 
  Direct return & GARCH & 3 & 0.749 \\ 
  Direct return & Naive window & 12 & 0.745 \\ 
  Direct return & Naive window & 3 & 0.736 \\ 
  Direct return & GARCH & 1 & 0.718 \\ 
  Factor model & Naive window & 6 & 0.715 \\ 
  Factor model & GARCH & 6 & 0.713 \\ 
  Factor model & GARCH & 3 & 0.710 \\ 
  Factor model & GARCH & 12 & 0.709 \\ 
  Factor model & Naive window & 3 & 0.709 \\ 
  Factor model & Naive window & 12 & 0.708 \\ 
  Direct return & Naive window & 1 & 0.698 \\ 
  Factor model & GARCH & 1 & 0.696 \\ 
  Factor model & Naive window & 1 & 0.689 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:All}
\end{table}


==> mean_kendall_for_All_app.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.762 \\ 
  Direct return & GARCH & 6 & 0.759 \\ 
  Direct return & Naive window & 6 & 0.751 \\ 
  Direct return & GARCH & 3 & 0.749 \\ 
  Direct return & Naive window & 12 & 0.745 \\ 
  Direct return & Naive window & 3 & 0.736 \\ 
  Direct return & GARCH & 1 & 0.718 \\ 
  Factor model & Naive window & 6 & 0.715 \\ 
  Factor model & GARCH & 6 & 0.713 \\ 
  Factor model & GARCH & 3 & 0.710 \\ 
  Factor model & GARCH & 12 & 0.709 \\ 
  Factor model & Naive window & 3 & 0.709 \\ 
  Factor model & Naive window & 12 & 0.708 \\ 
  Direct return & Naive window & 1 & 0.698 \\ 
  Factor model & GARCH & 1 & 0.696 \\ 
  Factor model & Naive window & 1 & 0.689 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'All'.} 
\label{tab:All}
\end{table}


==> mean_kendall_for_All_long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Dec 21 15:41:01 2021
\begin{table}[hb]
\centering
\begin{tabular}{lllr}
  \hline
Data/Model & Time modelling & q & Mean Kendall tau \\ 
  \hline
Direct return & GARCH & 12 & 0.586 \\ 
  Direct return & GARCH & 6 & 0.581 \\ 
  Direct return & Naiive window & 6 & 0.568 \\ 
  Direct return & GARCH & 3 & 0.568 \\ 
  Direct return & Naiive window & 12 & 0.553 \\ 
  Direct return & Naiive window & 3 & 0.551 \\ 
  Direct return & GARCH & 1 & 0.528 \\ 
  Factor model & Naiive window & 1 & 0.521 \\ 
  Factor model & GARCH & 1 & 0.521 \\ 
  Factor model & Naiive window & 3 & 0.520 \\ 
  Factor model & GARCH & 3 & 0.520 \\ 
  Factor model & Naiive window & 6 & 0.519 \\ 
  Factor model & GARCH & 6 & 0.519 \\ 
  Factor model & Naiive window & 12 & 0.518 \\ 
  Factor model & GARCH & 12 & 0.518 \\ 
  Direct return & Naiive window & 1 & 0.502 \\ 
   \hline
\end{tabular}
\caption{Mean Kendall tau for portfolio group 'All long'} 
\end{table}


==> mean_kendall_for_North.America.original.long.short.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & Naive window & 6 & 0.732 \\ 
  Direct return & GARCH & 6 & 0.731 \\ 
  Direct return & GARCH & 12 & 0.730 \\ 
  Direct return & Naive window & 3 & 0.728 \\ 
  Direct return & GARCH & 3 & 0.726 \\ 
  Direct return & Naive window & 12 & 0.722 \\ 
  Direct return & Naive window & 1 & 0.697 \\ 
  Direct return & GARCH & 1 & 0.696 \\ 
  Factor model & Naive window & 6 & 0.637 \\ 
  Factor model & Naive window & 12 & 0.633 \\ 
  Factor model & GARCH & 6 & 0.623 \\ 
  Factor model & Naive window & 3 & 0.622 \\ 
  Factor model & GARCH & 3 & 0.609 \\ 
  Factor model & GARCH & 12 & 0.606 \\ 
  Factor model & GARCH & 1 & 0.598 \\ 
  Factor model & Naive window & 1 & 0.590 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'North America original long/short'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:North.America.original.long.short}
\end{table}


==> mean_kendall_for_North.America.random.long.short.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & Naive window & 6 & 0.653 \\ 
  Direct return & GARCH & 6 & 0.645 \\ 
  Direct return & GARCH & 12 & 0.638 \\ 
  Direct return & Naive window & 12 & 0.638 \\ 
  Direct return & GARCH & 3 & 0.628 \\ 
  Direct return & Naive window & 3 & 0.626 \\ 
  Direct return & GARCH & 1 & 0.586 \\ 
  Direct return & Naive window & 1 & 0.570 \\ 
  Factor model & GARCH & 6 & 0.564 \\ 
  Factor model & Naive window & 6 & 0.564 \\ 
  Factor model & GARCH & 12 & 0.552 \\ 
  Factor model & Naive window & 12 & 0.551 \\ 
  Factor model & Naive window & 3 & 0.546 \\ 
  Factor model & GARCH & 3 & 0.545 \\ 
  Factor model & GARCH & 1 & 0.515 \\ 
  Factor model & Naive window & 1 & 0.510 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'North America random long/short'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:North.America.random.long.short}
\end{table}


==> mean_kendall_for_North.America.random.long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & Naive window & 3 & 0.707 \\ 
  Direct return & Naive window & 6 & 0.706 \\ 
  Direct return & GARCH & 3 & 0.705 \\ 
  Direct return & GARCH & 6 & 0.704 \\ 
  Factor model & GARCH & 6 & 0.702 \\ 
  Factor model & Naive window & 6 & 0.698 \\ 
  Direct return & GARCH & 12 & 0.696 \\ 
  Direct return & Naive window & 12 & 0.692 \\ 
  Factor model & GARCH & 12 & 0.687 \\ 
  Factor model & Naive window & 12 & 0.686 \\ 
  Factor model & GARCH & 3 & 0.680 \\ 
  Factor model & Naive window & 3 & 0.680 \\ 
  Direct return & GARCH & 1 & 0.667 \\ 
  Factor model & Naive window & 1 & 0.656 \\ 
  Factor model & GARCH & 1 & 0.655 \\ 
  Direct return & Naive window & 1 & 0.644 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'North America random long'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:North.America.random.long}
\end{table}


==> mean_kendall_for_Unrestricted.original.long.short.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.692 \\ 
  Direct return & Naive window & 12 & 0.676 \\ 
  Direct return & GARCH & 6 & 0.676 \\ 
  Direct return & Naive window & 6 & 0.671 \\ 
  Direct return & GARCH & 3 & 0.655 \\ 
  Direct return & Naive window & 3 & 0.649 \\ 
  Direct return & GARCH & 1 & 0.636 \\ 
  Direct return & Naive window & 1 & 0.626 \\ 
  Factor model & Naive window & 6 & 0.622 \\ 
  Factor model & GARCH & 12 & 0.616 \\ 
  Factor model & GARCH & 6 & 0.612 \\ 
  Factor model & Naive window & 12 & 0.610 \\ 
  Factor model & GARCH & 3 & 0.594 \\ 
  Factor model & Naive window & 3 & 0.593 \\ 
  Factor model & GARCH & 1 & 0.564 \\ 
  Factor model & Naive window & 1 & 0.551 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'Unrestricted original long/short'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:Unrestricted.original.long.short}
\end{table}


==> mean_kendall_for_Unrestricted.original.long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.575 \\ 
  Direct return & GARCH & 6 & 0.569 \\ 
  Direct return & GARCH & 3 & 0.558 \\ 
  Direct return & Naive window & 6 & 0.546 \\ 
  Direct return & Naive window & 3 & 0.538 \\ 
  Direct return & Naive window & 12 & 0.530 \\ 
  Direct return & GARCH & 1 & 0.512 \\ 
  Direct return & Naive window & 1 & 0.484 \\ 
  Factor model & Naive window & 6 & 0.447 \\ 
  Factor model & Naive window & 3 & 0.440 \\ 
  Factor model & GARCH & 6 & 0.439 \\ 
  Factor model & GARCH & 3 & 0.437 \\ 
  Factor model & GARCH & 12 & 0.433 \\ 
  Factor model & Naive window & 12 & 0.431 \\ 
  Factor model & GARCH & 1 & 0.414 \\ 
  Factor model & Naive window & 1 & 0.404 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'Unrestricted original long'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:Unrestricted.original.long}
\end{table}


==> mean_kendall_for_Unrestricted.random.long.short.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & Naive window & 6 & 0.592 \\ 
  Direct return & GARCH & 6 & 0.579 \\ 
  Direct return & GARCH & 12 & 0.579 \\ 
  Direct return & Naive window & 12 & 0.575 \\ 
  Direct return & GARCH & 3 & 0.556 \\ 
  Direct return & Naive window & 3 & 0.552 \\ 
  Factor model & GARCH & 6 & 0.543 \\ 
  Factor model & Naive window & 6 & 0.541 \\ 
  Factor model & GARCH & 12 & 0.534 \\ 
  Factor model & Naive window & 12 & 0.530 \\ 
  Factor model & Naive window & 3 & 0.524 \\ 
  Factor model & GARCH & 3 & 0.524 \\ 
  Direct return & GARCH & 1 & 0.492 \\ 
  Factor model & GARCH & 1 & 0.484 \\ 
  Direct return & Naive window & 1 & 0.480 \\ 
  Factor model & Naive window & 1 & 0.475 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'Unrestricted random long/short'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:Unrestricted.random.long.short}
\end{table}


==> mean_kendall_for_Unrestricted.random.long.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jan 17 15:08:39 2022
\begin{table}[ht]
\centering
\begin{tabular}{lllr}
  \toprule
Data/Model & Volatility modelling & q & avg($\tau$) \\ 
  \midrule
Direct return & GARCH & 12 & 0.551 \\ 
  Direct return & GARCH & 6 & 0.547 \\ 
  Direct return & GARCH & 3 & 0.535 \\ 
  Direct return & Naive window & 6 & 0.529 \\ 
  Direct return & Naive window & 3 & 0.517 \\ 
  Direct return & Naive window & 12 & 0.515 \\ 
  Direct return & GARCH & 1 & 0.485 \\ 
  Direct return & Naive window & 1 & 0.461 \\ 
  Factor model & Naive window & 6 & 0.436 \\ 
  Factor model & GARCH & 6 & 0.431 \\ 
  Factor model & Naive window & 3 & 0.430 \\ 
  Factor model & GARCH & 3 & 0.428 \\ 
  Factor model & GARCH & 12 & 0.422 \\ 
  Factor model & Naive window & 12 & 0.422 \\ 
  Factor model & GARCH & 1 & 0.406 \\ 
  Factor model & Naive window & 1 & 0.399 \\ 
   \bottomrule
\end{tabular}
\caption{Average Kendall tau for portfolio group 'Unrestricted random long'. q denotes the window length in months for the correlation structure (and also the variance structure for the naive window method)} 
\label{tab:Unrestricted.random.long}
\end{table}

